Language Evolution with Deep Learning

Computational modeling plays an essential role in the study of language emergence. It aims to simulate the conditions and learning processes that could trigger the emergence of a structured language within a simulated controlled environment. Several methods have been used to investigate the origin of our language, including agent-based systems, Bayesian agents, genetic algorithms, and rule-based systems. This chapter explores another class of computational models that have recently revolutionized the field of machine learning: deep learning models. The chapter introduces the basic concepts of deep and reinforcement learning methods and summarizes their helpfulness for simulating language emergence. It also discusses the key findings, limitations, and recent attempts to build realistic simulations. This chapter targets linguists and cognitive scientists seeking an introduction to deep learning as a tool to investigate language evolution.

==> buffer.tex <==
\section{brouillon}
    
    \subsection{Casting the Lewis Game as a MDP}
    
        \paragraph{Observation}  
            % one-hot, images, sounds, smell~\citep{Douwe}. 
            % We will explain in Sec Agent how to process this method with DL
        \paragraph{Action}
        \paragraph{Reward}
    
    \subsection{Overfitting and Generalization}
    % Introduce the concept of valid/test set

    \subsection{Extension of the game ?}



\section{Modeling agents with Deep Networks}
\label{sec:agent}

    \subsection{Deep Learning Basics.}
        % background history
        \paragraph{Neural Networks}
        \paragraph{Network for Spatial Input}
        \paragraph{Network for Temporal Input}
        \paragraph{How to combine Neural Modules}
    
    \subsection{Modelling a communication agent}
        \paragraph{Language generator}
        \paragraph{Language perception}
        \paragraph{Environment perception}
        \paragraph{Module act}

\section{Updating the Agent}
\label{sec:update}

% \begin{itemize}
%     \item General description of gradient descent, etc.
%     \item Continuous latent space
%     \item Discrete latent space 1: gumbel softmax
%     \item Discrete latent space 2: REINFORCE
% \end{itemize}

    \subsection{Loss Definition.}
        \paragraph{Loss Objective}
        \paragraph{General description of gradient descent}
        \paragraph{Backpropagation}
        \paragraph{Optimizer}

    \subsection{Training the Language Model}
    
    \subsection{Training the Action Module}
        % One-step Cross entropy
        % N-step
        
    \subsection{The Gumbel-softmax trick}
    
    \subsection{Advanced Learning method}
    % Improving the RL algorithm: KL, entropy




\subsection{Taxonomy}

\subsubsection{Recovering language universals}

\begin{itemize}
    \item Compositionality and generalization
    \item Zipf Law
    \item Other ? Word order ?
\end{itemize}

\subsubsection{Iterated learning: a successful application of language evolution theory to machine learning (scale in time)}

\subsubsection{Scaling up simulations with populations (scale in space)}

\begin{itemize}
    \item Emergent communication at scale
    \item Community size
    \item Communication graph structure
\end{itemize}




%%% EX DESIGNING THE GAME

\subsection{Designing the game \mathieu{(rajouter des figures limpides)}}
\label{subsec:design_env}

The practitioner first aims at designing the game. The game is fully characterized by (1) an \textit{environment} in which the agents play the game, (2) a \textit{task} agents have to solve, (3) a \textit{communication channel} in which agents can communicate. Beyond the game itself, this modeling step crucially shapes the communication challenge: on the one hand, the environment and task determines the quantity of information agents must communicate about; on the other hand, the communication channel limits the maximum expressivity of agents' languages.

\subsubsection{Environment (States) \mathieu{clarifier}}

During the game, agents have access to states, or observations provided by an \textit{environment}. In Lewis Games, the receiver have a partial view of those states and the sender must complete this view to help the receiver achieve the task. 
Commonly in standard neural network experiments, the environment is either a dataset whose elements are given to the agents or a simulated environment in which agents have access to different pieces of information. For example, the environment could be a dataset of images or a 2D grid in which the sender and receiver can navigate.

\subsubsection{Task \mathieu{(être plus clair sur des exemples classiques)}}
\label{subsec:task}

During the game, agents should communicate and act in order to solve a \textit{task}.  We distinguish two types of tasks:

\begin{itemize}
    \item \textit{Pure Communication task}: the task can fully be solved if the receiver correctly interpret the content of sender's messages. For example, such task could be the discrimination by the receiver of an object seen by the sender among a set of distractors.
    \item \textit{Partial communication task}: the interpretation by the receiver of the content of sender's messages alone is not enough to solve the task. The receiver should then use both the information provided by the sender and the information available in the environment to solve the task. For example, such task could be the navigation toward a goal into a 2D grid where the information about the goal is only accessible by the sender. 
\end{itemize}

The success of the task is quantified by a \textit{reward function}. The reward function maps the actions of the receiver and the states of the environment to a real number. For example, in the discrimination task, a common \textit{reward function} is the function equal to $1$ if the receiver points to the correct object among the set of distractors, $0$ otherwise. For the navigation task, a potential reward function is the function equal to $1$ if the receiver reaches its goal, $0$ otherwise.

\subsubsection{Communication channel}
\label{subsec:communication_channel}

In order to solve the task into the environment, the agents are given a \textit{communication channel} through which they can communicate.
In standard emergent communication settings \mathieu{REF}, communication protocols are discrete and recursive \footnote{Note that some work consider continuous communication protocol, \mathieu{à compléter}}{} \mathieu{REF} meaning that a message is a sequence of symbols, each taken from a vocabulary. The communication channel is thus parameterized by two factors:
\begin{itemize}
    \item The \textit{vocabulary size}: the maximum number of different symbols an agent can use.
    \item The \textit{maximum length}: the maximum length of a message an agent can send.
\end{itemize}

Formally, a message is thus a sequence: $m=(m_{1},...,m_{L})$ where each message belongs to a vocabulary $V$ of size $|V|$ and $L$ is the length of the message which is maximally equal to $max\_length$ the maximum length of a message.

\subsubsection{Designing the game affects the information complexity/expressivity ratio}
\label{subsec:complexity}

During a communication game, the sender should identify the information provided by the environment that is useful for the receiver to solve the task and communicate about it through the communication channel. As such, the communication channel is an information bottleneck: agents should communicate through a channel with a limited expressivity capacity. The design of the game crucially imposes the tightness of the information bottleneck and thus the difficulty of building a communication protocol:

\begin{itemize}
    \item The \textbf{environment} defines the maximum quantity of information an agent can communicate about. For example, if the environment is composed of objects characterized by a color among $5$ possible colors and a shape among $5$ possible shapes, the total number of combination is equal to $25$. 
    \item The \textbf{task} reduces the quantity of information to a smaller quantity that is useful for the receiver to solve the task. For example, using the previous example, if the task is the reconstruction by the receiver of the color of an object seen by the sender, the task reduces the quantity of information to be transmitted to the color of the objects, ie. to $5$ possibilities.
    \item The \textbf{communication channel} introduces a maximum expressivity capacity, ie. the maximum quantity of information the sender can transmit to the receiver. With the definition of the communication channel proposed in this chapter, the expressivity capacity is fully determined by the vocabulary size $|V|$ and the maximum length $max\_length$. Indeed, the total number of possible messages is equal to $|V|^{max\_length}$.
\end{itemize}

The comparison between the complexity induced by the environment and the task and the expressivity capacity of the communication channel is key. Using previous example, if the total number of possible messages is equal to $4$, agents cannot communicate about $5$ different colors. When modeling the game, one should carefully choose the parameters affecting the ratio between the complexity and expressivity.




\subsection{Formalizing the game as a machine learning problem}
\label{subsec:formalism_game}

% Idéalement il faudrait passer en 3 paragraphes:
% 1. Markov Game
% 2. Policies
% 3. Optim pb
% Pour qu'ensuite il y ait un echo dans toutes les parties suivantes

Markov Games~\citep{littman1994markov} offer a unified mathematical framework to study Lewis Games where the two agents aim at optimizing a communication outcome partly determined by the agents and partly random. 

\paragraph{Framing Lewis Games as Markov Games}
We first aim at framing Lewis Games as Markov Games. To ease comprehension, we will use the case of the Visual Discrimination Game as a thread example (see Table~\ref{tab:taxo_tasks}). %In this game, the sender in observing an image. It then communicates a message to the receiver, that has to recover this original image among a set of $N$ images.
\\

Taking Markov Games formalism, Lewis Games with two players can be defined as a tuple:
\begin{align*}      (\mathcal{S},\mathcal{A}_{\sender},\mathcal{A}_{\receiver},\mathcal{P},\mathcal{R})
\end{align*}

where: 
\begin{itemize}
    \item $\mathcal{S}$ is a set of states. It describes all the possible configuration of the game at one instant. Besides, each agent may only observe a snapshot of this state, which is described by the two observations $o_{\sender}$ and $o_{\receiver}$. 
    %example
    In the Visual Discrimination Game, the sender observation is an image and the receiver observation is both the set of $N$ images and the message sent by the sender.
    %
    \item $\mathcal{A}_{\sender}$ and $\mathcal{A}_{\receiver}$ are the set of actions for the sender and the receiver. In the context of Lewis Games, sender's actions $\mathcal{A}_{\sender}$ are the messages the sender can send. %To ease reading, we will next denote $\mathcal{A}_{sender}$ by $\mathcal{M}$ and a message sent by the sender $m$. 
    Note that Lewis Games are turn-based Markov Games, meaning that the two agents always act one after the other.
    %example
    In the Visual Discrimination Game, the set of sender actions $\mathcal{A}_{\sender}$ is the set of messages the sender can send to the receiver ; actions of the receiver $\mathcal{A}_{\receiver}$ are the different choices of images when trying to recover the image seen by the sender.
    %
    %\item $\mathcal{O}_{sender}$ and $\mathcal{O}_{receiver}$ are the functions that map all the information available in the environment to observations of the two agents $\mathcal{o}_{sender}$ and $o_{receiver}$. It can be either the states, partial view of the states or the actions of the other agents. %example
    %In the Visual Discrimination Game, the state $\mathcal{s}$ is the set of $N$ images, $o_{sender}$ is a random image among those $N$ images and $o_{receiver}$ is both full observation of the state $s$ and the action of the sender, i.e the message sent.
    %
    \item $\mathcal{P}:(\mathcal{S}\times\mathcal{A}_{\sender}\times\mathcal{A}_{\receiver},\mathcal{S}) \to [0,1]$ is the probability of reaching state $s' \in \mathcal{S}$ when agents perform actions $a_{\sender} \in \mathcal{A}_{\sender}$ and $a_{\receiver} \in \mathcal{A}_{\receiver}$ while being in the state $s \in \mathcal{S}$. 
    %example
    In the Visual Discrimination Game, the probability $\mathcal{P}$ is uniform and thus does not take any role. $\mathcal{P}$ is useful when modeling a complex environment that depends on agents' actions.
    %
    \item $\mathcal{R}:(\mathcal{S},\mathcal{A}_{\sender},\mathcal{A}_{\receiver}) \to \mathbb{R}$ is a reward function that returns a common pay-off for the two agents when the agents perform actions $a_{\sender} \in \mathcal{A}_{\sender}$ and $a_{\receiver} \in \mathcal{A}_{\receiver}$ while both being the state $s \in \mathcal{S}$. 
    %example
    In the Visual Discrimination Game, the reward could be the function equal to $0$ when the receiver picks up the correct image seen by the sender, $0$ otherwise.
    %
    %\item $\mathcal{I}:\{0,1\}\to [0,1]$ : is the probability that the sender and receiver perform an action at the current instance of the game. 
    %example
    %In the Visual Discrimination Game and more broadly in 2 players Lewis Games, there is an alternation between the sender action and the receiver action: first the sender sends a message, second the receiver tries to decode the message to achieve the task.
\end{itemize}

\paragraph{Sender's set of actions is the language space} In Lewis Games, sender's actions take a particular form: 

sender's task is to define a mapping $\pi_{sender}$ between observations $o_{sender}$ and messages $m$. This mapping is a communication protocol that we further name \textit{emergent language}.

\paragraph{Lewis Games as an decision-making problem}

Lewis Games are decision making problems: the sender and receiver must agree on a protocol to collect the maximum common reward. The way the sender and receiver behave with each other and their environment is characterized by action policies, i.e. decision-making rules:
\begin{itemize}
    \item $\pi_{\sender}$ is sender's policy, i.e. the message $m$ sent by the sender when observing $o_{\sender}$.
    % Visual discrimination game
    In the Visual Discrimination Game, $\pi_{\sender}(m|o_{\sender})$ is the probability of sending $m$ when observing $o_{\sender}$.
    \item $\rho_{\reicever}$ is receiver's policy, i.e. the action taken $a_{\receiver}$ by the receiver when observing $o_{\receiver}$, its view of the state $s$ and sender's message $m$.
    % Visual discrimination game
    In the Visual Discrimination Game, $\rho_{\reicever}(a_{\receiver}|o_{\receiver})$ is the probability of picking an image when observing the set of $N$ images and sender's message.
\end{itemize}

 The goal of the two agents is to agree on a communication protocol that maximises the expected common reward. In Section~\ref{subsec:design_optim}, we translate this statement into an optimization problem that could be solve using machine learning.


 \subsection{Designing the game}
\label{subsec:design_env}

Once a specific variant of the Lewis Game is chosen, the implementation requires to define each of the elements of the tuple
\begin{align*}
    (\mathcal{S},\mathcal{A}_{\sender},\mathcal{A}_{\receiver},\mathcal{P},\mathcal{R})
\end{align*} 
In practice, the modelling process involves determining (1) the task that the agents need to complete, including the set of states $\mathcal{S}$, receiver's actions $\mathcal{A}_{receiver}$, the transition matrix $\mathcal{P}$ and the reward $\mathcal{R}$; (2) the communication channel, including the set of messages the sender can send $\mathcal{M}$. This modelling step is even more important because it determines the relationship between the complexity of the task and the maximum expressiveness of the communication channel.


In Figure~\ref{fig:tasks}, we derive a genealogy of the different types of Lewis Games and their corresponding references in the neural emergent communication literature. The tree is drawn according to two criteria:
\begin{itemize}
    \item Making the communication successful is the only goal of the task: it distinguishes between pure communication tasks and partial communication tasks. In pure communication task, the transition matrix $\mathcal{P}$ does not take any role, while in partial communication task $\mathcal{P}$ shapes the dynamics of the environment and increases the complexity of the game.
    \item The states $\mathcal{S}$ should be entirely communicated by the sender: it distinguishes between tasks where the emergent languages should be expressive with respect to the full set of states and the tasks where the expressivity challenge is reduced.
\end{itemize}
% \begin{itemize}
%     \item Games where the goal is the success of the communication (pure communication task).% In this case, the environment is merely composed of a dataset of objects agents should communicate about: $\mathcal{S}$ is a dataset of objects, $\mathcal{P}$ is a uniform matrix without any impact, $\mathcal{R}$ reward the success of the communication.
%     \item Games where agent's communication is a mean to achieve a task in a complex environment (partial communication task). In this case, the receiver must both decipher sender's messages but also understand its environment to solve the task.%In this case, $\mathcal{S}$, $\mathcal{P}$ defines the dynamic of the environment and $\mathcal{R}$ rewards not only the communication bu
% \end{itemize}



\paragraph{The communication channel} The sender interacts with the receiver agent through a \textit{communication channel}. In standard emergent communication settings~\citep{lazaridou2018emergence,chaabouni2019anti,kottur2017natural,li2019ease,chaabouni2022emergent,rita2022on}, communication protocols are discrete and recursive\footnote{Note that some work consider continuous communication protocol~\citep{tieleman2019shaping} \mathieu{compléter}}{} meaning that a message is a sequence of symbols, each taken from a vocabulary. 
% % exemple
For example, if the vocabulary is a set of $3$ symbols $[a,b,c]$, messages could be sequences like: $'aacba'$ or $'cbabbca'$.
% % formalisme
More generally, the communication channel is parameterized by two factors:
\begin{itemize}
    \item The \textit{vocabulary size}: the maximum number of different symbols an agent can use.
    \item The \textit{maximum length}: the maximum length of a message an agent can send.
\end{itemize}

The message is then a sequence: $m=(m_{1},...,m_{L})$ with a defined maximum length $max\_length$  where each message belongs to a vocabulary $V$ of size $|V|$.

\paragraph{The information ratio} The parametrization of the game is key as it shapes a ratio between the complexity of the task and the expressiveness of the communication channel. On the one hand, the environment is characterized by a given complexity, induced by the states $\mathcal{S}$ and the transition matrix $\mathcal{P}$. This complexity is reduced by the difficulty of the task, characterized by receiver's actions $\mathcal{A}_{receiver}$ and the reward $\mathcal{R}$. On the other hand, the communication channel has a given size that shapes the maximum expressiveness of the sender. From the point of view of the sender, this information ratio shapes a communication bottleneck that constraints the communication protocol that emerges.
%
For example, in the Visual Discrimination Game, the set of images (states $\mathcal{S}$) to communicate imposes a large complexity. This complexity is reduced by the task (characterized by $\mathcal{A}_{receiver}$ and $\mathcal{R}$), which is discriminating an image among a set of $N$ images. This complexity should be compared to the size of the communication channel. In the discrete and recursive case, the size of the communication channel is equal to $|V|^{max\_length}$.









\section{Training agents to solve Lewis games}
\label{sec:implementing_Lewis_Game}

In the section, we present all the concepts and methods required to design a Lewis game with neural networks optimized by machine learning. First, we describe in practice how to implement the game (Sec.~\ref{subsec:design_env}). Second, we build artificial communicative agents with neural networks (Sec.~\ref{subsec:design_agents}). Third, we present the basics of machine learning optimization and apply them to the learning of the communication agents (Sec.~\ref{subsec:design_optim}).

%focus on deep reinforcement learning methods, formalizing (i) how the tasks is formally defined (Sec.~\ref{sec:env}), (ii) how the agents are modelled (Sec.~\ref{sec:agent}), (iii) and how the agents are updated (Sec.~\ref{sec:update}).

% Nouveau plan potentiel:
% 1. Formalism
% 2. Designing the env
% 3. Designing the agents
% 4. Optimizing the game


\subsection{Designing the game}
\label{subsec:design_env}

Once a specific variant of the Lewis Game is chosen, the implementation requires to define each of the elements of the tuple
\begin{align*}
    (\mathcal{S},\mathcal{A}_{\sender},\mathcal{A}_{\receiver},\mathcal{P},\mathcal{R})
\end{align*} 
%In practice, the modelling process involves determining (1) the task that the agents need to complete, including the set of states $\mathcal{S}$, receiver's actions $\mathcal{A}_{receiver}$, the transition matrix $\mathcal{P}$ and the reward $\mathcal{R}$; (2) the communication channel, including the set of messages the sender can send $\mathcal{M}$. This modelling step is even more important because it determines the relationship between the complexity of the task and the maximum expressiveness of the communication channel.

\paragraph{The states $\mathcal{S}$} \mathieu{TO DO}

\paragraph{Sender's actions $\mathcal{A}_{\sender}$} Sender's actions are messages sent to the receiver. In standard emergent communication settings~\citep{lazaridou2018emergence,chaabouni2019anti,kottur2017natural,li2019ease,chaabouni2022emergent,rita2022on}, communication protocols are discrete and recursive\footnote{Note that some work consider continuous communication protocol~\citep{tieleman2019shaping} \mathieu{compléter}}{} meaning that a message is a sequence of symbols, each taken from a vocabulary. 
% % exemple
For example, if the vocabulary is a set of $3$ symbols $[a,b,c]$, messages could be sequences like: $'aacba'$ or $'cbabbca'$.
% % formalisme
More generally, the communication channel is parameterized by two factors:
\begin{itemize}
    \item The \textit{vocabulary size}: the maximum number of different symbols an agent can use.
    \item The \textit{maximum length}: the maximum length of a message an agent can send.
\end{itemize}

The message is then a sequence: $m=(m_{1},...,m_{L})$ with a defined maximum length $max\_length$  where each message belongs to a vocabulary $V$ of size $|V|$.

\paragraph{Receiver's actions $\mathcal{A}_{\receiver}$}  \mathieu{TO DO}

\paragraph{Transition matrix $\mathcal{P}$} Transition matrix characterizes the dynamic of the environment in response the receiver's actions. 

\paragraph{The reward}  \mathieu{TO DO}

% \begin{itemize}
%     \item Games where the goal is the success of the communication (pure communication task).% In this case, the environment is merely composed of a dataset of objects agents should communicate about: $\mathcal{S}$ is a dataset of objects, $\mathcal{P}$ is a uniform matrix without any impact, $\mathcal{R}$ reward the success of the communication.
%     \item Games where agent's communication is a mean to achieve a task in a complex environment (partial communication task). In this case, the receiver must both decipher sender's messages but also understand its environment to solve the task.%In this case, $\mathcal{S}$, $\mathcal{P}$ defines the dynamic of the environment and $\mathcal{R}$ rewards not only the communication bu
% \end{itemize}



% \paragraph{The communication channel} The sender interacts with the receiver agent through a \textit{communication channel}. In standard emergent communication settings~\citep{lazaridou2018emergence,chaabouni2019anti,kottur2017natural,li2019ease,chaabouni2022emergent,rita2022on}, communication protocols are discrete and recursive\footnote{Note that some work consider continuous communication protocol~\citep{tieleman2019shaping} \mathieu{compléter}}{} meaning that a message is a sequence of symbols, each taken from a vocabulary. 
% % % exemple
% For example, if the vocabulary is a set of $3$ symbols $[a,b,c]$, messages could be sequences like: $'aacba'$ or $'cbabbca'$.
% % % formalisme
% More generally, the communication channel is parameterized by two factors:
% \begin{itemize}
%     \item The \textit{vocabulary size}: the maximum number of different symbols an agent can use.
%     \item The \textit{maximum length}: the maximum length of a message an agent can send.
% \end{itemize}

% The message is then a sequence: $m=(m_{1},...,m_{L})$ with a defined maximum length $max\_length$  where each message belongs to a vocabulary $V$ of size $|V|$.

% \paragraph{The information ratio} The parametrization of the game is key as it shapes a ratio between the complexity of the task and the expressiveness of the communication channel. On the one hand, the environment is characterized by a given complexity, induced by the states $\mathcal{S}$ and the transition matrix $\mathcal{P}$. This complexity is reduced by the difficulty of the task, characterized by receiver's actions $\mathcal{A}_{receiver}$ and the reward $\mathcal{R}$. On the other hand, the communication channel has a given size that shapes the maximum expressiveness of the sender. From the point of view of the sender, this information ratio shapes a communication bottleneck that constraints the communication protocol that emerges.
% %
% For example, in the Visual Discrimination Game, the set of images (states $\mathcal{S}$) to communicate imposes a large complexity. This complexity is reduced by the task (characterized by $\mathcal{A}_{receiver}$ and $\mathcal{R}$), which is discriminating an image among a set of $N$ images. This complexity should be compared to the size of the communication channel. In the discrete and recursive case, the size of the communication channel is equal to $|V|^{max\_length}$.


% \subsubsection{Framing Lewis Games as MDPs}

% The problem of building a communication protocol through interaction is a decision making problem where the decision maker is a speaker agent who should build the language that best optimizes a communication reward that varies depending on a listener agent understanding. Lewis Games can be framed as Markov Decision process. In what follows, we match the $4$ components of the MDP to aspects of the game and define the optimization problem.

% \paragraph{State space}

% % expli
% During the game, agents have access to states, or observations of their environment \textit{environment}. In Lewis Games, the receiver have a partial view of those states and the sender must complete this view to help the receiver achieve the task. 
% % example
% Commonly in standard neural network experiments, the environment is either a dataset whose elements are given to the agents or a simulated environment in which agents have access to different pieces of information. For example, the environment could be a dataset of images or a 2D grid in which the sender and receiver can navigate.
% % formalism

% \paragraph{Action space}
% \label{subsec:communication_channel}



% % expli
% In Lewis Games, the sender agent can interact with the receiver agent through a \textit{communication channel}. The action space is therefore the entire set of messages the sender agent can send. In standard emergent communication settings~\citep{lazaridou2018emergence,chaabouni2019anti,kottur2017natural,li2019ease,chaabouni2022emergent,rita2022on}, communication protocols are discrete and recursive\footnote{Note that some work consider continuous communication protocol~\citep{tieleman2019shaping} \mathieu{compléter}}{} meaning that a message is a sequence of symbols, each taken from a vocabulary. 
% % exemple
% For example, if the vocabulary is a set of $3$ symbols $[a,b,c]$, messages could be sequences like: $'aacba'$ or $'cbabbca'$.
% % formalisme
% More generally, the communication channel is parameterized by two factors:
% \begin{itemize}
%     \item The \textit{vocabulary size}: the maximum number of different symbols an agent can use.
%     \item The \textit{maximum length}: the maximum length of a message an agent can send.
% \end{itemize}

% Formally, a message is then a sequence: $m=(m_{1},...,m_{L})$ where each message belongs to a vocabulary $V$ of size $|V|$ and $L$ is the length of the message which is maximally equal to $max\_length$ the maximum length of a message.

% \subsubsection{Designing the game affects the information complexity/expressivity ratio}
% \label{subsec:complexity}

% During a communication game, the sender should identify the information provided by the environment that is useful for the receiver to solve the task and communicate about it through the communication channel. As such, the communication channel is an information bottleneck: agents should communicate through a channel with a limited expressivity capacity. The design of the game crucially imposes the tightness of the information bottleneck and thus the difficulty of building a communication protocol:

% \begin{itemize}
%     \item The \textbf{environment} defines the maximum quantity of information an agent can communicate about. For example, if the environment is composed of objects characterized by a color among $5$ possible colors and a shape among $5$ possible shapes, the total number of combination is equal to $25$. 
%     \item The \textbf{task} reduces the quantity of information to a smaller quantity that is useful for the receiver to solve the task. For example, using the previous example, if the task is the reconstruction by the receiver of the color of an object seen by the sender, the task reduces the quantity of information to be transmitted to the color of the objects, ie. to $5$ possibilities.
%     \item The \textbf{communication channel} introduces a maximum expressivity capacity, ie. the maximum quantity of information the sender can transmit to the receiver. With the definition of the communication channel proposed in this chapter, the expressivity capacity is fully determined by the vocabulary size $|V|$ and the maximum length $max\_length$. Indeed, the total number of possible messages is equal to $|V|^{max\_length}$.
% \end{itemize}

% The comparison between the complexity induced by the environment and the task and the expressivity capacity of the communication channel is key. Using previous example, if the total number of possible messages is equal to $4$, agents cannot communicate about $5$ different colors. When modeling the game, one should carefully choose the parameters affecting the ratio between the complexity and expressivity.

\subsection{Designing communicative agents with neural networks}
\label{subsec:design_agents}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{buffer_figures/agent_draft_figure.png}
    \caption{Agent design for communication games. (a) General view an agents and its interaction with environment and message space ; (b) Agent modelling as functional modules: a \textbf{perception module} that maps states to a \textit{perceptual representation} ; a \textbf{generation module} that maps the \textit{perceptual representation} as a message ; an \textbf{understanding module} that maps a message to an internal \textit{message representation} ; an \textbf{action module} that maps the \textit{message representation} to an action ; \mathieu{(c) Examples of neural nets with inputs and outputs TO DO}}
    \label{fig:designing_agents}
\end{figure}

We now need to model communicative agents $\pi_{\sender}$ and $\rho_{\receiver}$. In Section~\ref{subsubsec:functional_modules}, we show how an artificial agent can be decomposed into functional modules that will allow it to interact with its environment and other agents. In Section~\ref{subsubsec:neural_nets}, we give a definition of a neural network and show that neural networks can be used to parameterize the functional modules.

\subsubsection{Designing a communicative agent as functional modules}
\label{subsubsec:functional_modules}

As shown in Figure~\ref{fig:designing_agents}, a communicative agent should be able to interact with:
\begin{itemize}
    \item \textit{Its environment} by passively perceiving a stimulus or actively taking an action that will impact the environment ;
    \item \textit{Another agent} through a message space by passively interpreting or actively sending a message.
\end{itemize}

As a result, an agent can minimally be modelled by 4 functional modules: a \textbf{perception module} that maps a stimulus received from the environment to an internal \textit{perceptual representation}, a \textbf{generation module} that generates a message based on the internal \textit{perceptual representation}, an \textbf{understanding module} that takes a message a build an internal \textit{message representation} and an \textbf{action module} that maps the internal \textit{message representation} to an action in the environment.

When acting as a sender (resp. receiver), only two of those modules are involved: the perception and generation module (resp. the understanding and action module).

\subsubsection{From functional modules to neural networks}
\label{subsubsec:neural_nets}

We now aim at designing an agent as a neural network. (1) We define neural networks and (2) we describe how each functional module can be designed as a neural network.

\paragraph{Definition of a neural network} A Neural network is a biologically inspired system used to parameterize functions or probability distributions. A neural network is thus an application that maps inputs to outputs. The term \textit{neural} comes from the specific form of this mapping function: a neural network is composed of a network of connected nodes gathered in layers. Each node of a layer is composed of a set of weights and a threshold: each node receives a signal from the nodes of the previous layer on which it applies a linear transformation with its weights. If the resulting value is above the threshold, the node is activated and the weighted result is sent to the following connected nodes. Each node then mimics the behavior of neurons in biological systems.


Formally, we denote by $x$ the input of the neural network belonging to the input space $\mathcal{X}$ and $y$ its corresponding output in an output space $\mathcal{Y}$ and $\theta$ the set of all weights in the network. A neural network $f_{\theta}$ is then merely a mapping function of inputs $x \in \mathcal{X}$ to outputs $y$ of $\mathcal{Y}$:

\begin{align}
    y = f_{\theta}(x)
    \label{eq:NN}
\end{align}

Deep learning methods study the design of the \textit{architecture} of those neural networks and how to learn the best weights $\theta$ based on a limited number of input/output examples $(x,y)$: the \textit{training set}. The success of deep learning comes from the unprecedent success of its applications to unsolved problems (\mathieu{REF}). 

In what follows, we present standard ways of designing the modules of a communicative agents with neural networks. In any case, the choice of architecture for the neural network is motivated by the structure of the input data.

\paragraph{Building a perception module as a neural network} The perception module maps the environment state, or stimulus, the agent perceive into an internal representation. Taking Eq.~\ref{eq:NN}, $f_{\theta}$ is the perception module that takes the environmental state $x$ as input and maps it to the internal representation $y$.
The choice of architecture is closely related to the structure of the input state $x$. We summarize some of data structures and their corresponding neural net architectures in Table \ref{tab:architectures}

\bigbreak
Let's take the example of visual input states. In this case, the perception module should be chosen in order to build meaningful image representations. A well-suited class of neural networks is \textit{Convolutional Neural Networks (CNN)}. Convolutional networks are inspired by the visual cortex of animals: each node of the neural network is specialized on a restricted region of the visual field as it is observed for visual cortical neurons. A Convolutional network is mainly composed of convolutional filters that work at different scales of the image. This allows to capture specific features of the image, e.g. edges, colors, details. The output $y$ of the network is a vector of a chosen dimension, called \textit{embedding}, that we can use as the agent \textit{perceptual representation}. This representation captures in a high-dimension vector the information about the input image $x$.

\begin{table}[t]
\begin{center}
\begin{tabular}{c | c } 
 \hline
 Data structure & Neural net architectures \\ [0.5ex] 
 \hline \hline
 Multi-layer perceptron (MLP) & scalars \\
 Look-up table & tabular \\
 Convolutional Neural networks (CNN) & images, speech \\
 Recurrent neural networks (RNN, LSTM, GRU) & text, sequences \\ 
 Transformers & text, sequences, images, speech \\ 
 Graph Neural networks (GNN) & graphs \\
 \hline
\end{tabular}
\end{center}
\caption{Examples of different neural network architectures and the data structures they are used with}
\label{tab:architectures}
\end{table}

\paragraph{Building a generation module as a neural network} The generation module maps the \textit{internal representation} to messages, i.e. a sequence of discrete symbols. \mathieu{TO DO}

\paragraph{Building an understanding module as a neural network} \mathieu{TO DO}

\paragraph{Building an action module as a neural network} \mathieu{TO DO}

\paragraph{End to end agents: going beyond modules}

\subsubsection{The sender and the receiver}
\label{subsubsec:sender_receiver}

\subsection{Optimizing the game}
\label{subsec:design_optim}

As described in Section \label{sec:Lewis_and_ML}, the ultimate goal of the agents is to maximize their reward given a task, which constitutes their machine learning problem. This Section aims at introducing the optimization tools that solves a machine learning problem and how those tools apply to the communication game. 

In this section, we will show (1) how to formalize Section \label{subsec:formalism_game}'s decision-making problem of the communication game as an optimization problem, (2) how to train agent to optimize the problem, (3) the different types of training regimes in machine learning.

\subsubsection{Optimizing a machine learning problem}

\paragraph{Measuring the performance $P$: the loss function}

\mathieu{Partir de la notion générale de loss et aboutir à l'optim de reward dans notre pb}

In order to make a program learn, the practitioner has to define a score that measures the success of the program $f_{\theta}$ on the task $T$ when experiencing $E$. This score is called the \textit{loss function} $\mathcal{L_{\theta}}$. Note that the loss function is averaged on the experience $E$ ($\mathcal{L}_{\theta} = \mathbb{E}_{E}l_{\theta}$). The goal of training a model is then to find the set of model parameters $\theta$ that minimize the loss function given the experience $E$:

\begin{align}
    \min_{\theta} \mathcal{L}_{\theta}
    \label{eq:min_pb}
\end{align}

\\

The choice of a loss function depends on the specific task that the model is being trained for. For example, in a classification task (e.g. object selection, attribute reconstruction), the loss function might measure the difference between the predicted class probabilities and the true class labels. In a regression task (e.g. pixel reconstruction), the loss function might measure the difference between the predicted values and the true values. The specific form of the loss function is key as it has a significant impact on the performance of the trained model.

\paragraph{Learning to optimize the performance $P$: the gradient descent}

For a computer program $f_{\theta}$, learning means improving with respect to to the optimization problem \ref{eq:min_pb}. Among all the ways of performing this optimization problem, \textit{gradient descent} methods are the most successful approaches. The gradient descent is an iterative optimization algorithm that attempts to find the minimum of a function by following the negative gradient of the function. The model parameters $\theta$ are updated at each iteration in the direction that reduces the value of the loss function. The size of the update is determined by a hyperparameter called the learning rate. The update is written: 

\begin{align}
    \theta_{n+1} = \theta_{n} - \eta \nabla_{\theta}\mathcal{L}_{\theta}(\theta_{n})
\end{align}

where $\theta_{n}$ is the model parameters at step $n$, $\theta_{n+1}$ is the model parameters at step $n+1$, $\nabla_{\theta}\mathcal{L}_{\theta}$ the gradient of $\mathcal{L}$ and $\eta$ the learning rate.

\begin{tcolorbox}
Using gradient descent yields several challenges:

\begin{itemize}
    \item \textbf{Estimating the gradient}: In practice, computing the gradient $\nabla_{\theta}\mathcal{L}_{\theta}$ at every step is impossible as it would require to compute the error over all the experience $E$. In practice, we tackle this issue by using the \textit{stochastic gradient descent} which is a variant a gradient descent for which the gradient $\nabla_{\theta}\mathcal{L}_{\theta}$ is approximated at each step using a small subset, called batch, of the experience $E$. This batch should be large enough to ensure that the estimated gradient fairly approximates the true gradient $\nabla_{\theta}\mathcal{L}_{\theta}$. The practitioner should tune the size of the batch.
    \item \textbf{Adjusting the learning rate}: The learning rate $\eta$ controls the amplitude of the update at each step. Training dynamics are largely impacted by the choice of this parameter. Qualitatively, $\eta$ can be interpreted as a resolution parameter. On the one hand, if $\eta$ is too small, the algorithm captures very small variations of the loss function. However, the training is very slow as $\theta_{n+1}$ will be very close to $\theta_{n}$ for each iteration. On the other hand, if $\eta$ is too big, the training is fast but the algorithm cannot capture fine variations of the loss function and the estimation of model parameters minimizing $\mathcal{L}_{\theta}$ is imprecise. In practice, practitioners get ride of this issue by using the \textit{Adam optimizer} which is a variant of stochastic gradient descent that uses an adaptive learning rate, which means that the learning rate is automatically adjusted based on the dynamics of the training. 
\end{itemize}
\end{tcolorbox}

\paragraph{Learning from experience $E$: the generalization issue} Previously presented tools allow to optimize the performance $P$ when experiencing $E$ during the training. However, this performance score on the training experience is not necessarily indicative of the performance on new, unseen experience. It is thus necessary to distinguish (1) the training experience $E_{train}$ and the corresponding performance $P_{train}$ of the model on $E_{train}$, (2) the test experience $E_{test}$ and the corresponding performance $P_{test}$ of the model on $E_{test}$. $P_{test}$ indicates how well the model generalizes. In standard machine learning training, 3 regimes are observed:

\begin{itemize}
    \item \textbf{Underfitting}: When the model is undertrained, it is unable to have good performance $P$ neither on the training and test experience. $P_{train}$ and $P_{test}$ are bad.
    \item \textbf{Generalization}: During training, there is a time when both the both $P_{train}$ and $P_{test}$ are good. It may not be the optimal performance $P_{train}$ that could be achieved on $E_{train}$ but it is a good compromise to generalize well.
    \item \textbf{Overfitting}: When the model is overtrained, it reaches very good performances $P_{train}$ on $E_{train}$ but performances $P_{test}$ on $E_{test}$ are bad: the model overfits on the training experience.
\end{itemize}

The main challenge of machine learning is to find the right balance between under and overfitting to reach the generalization regime. Several methods are commonly used including regularization techniques and early stopping, which consists in introducing an evaluation experience $E_{eval}$ for which the performance $P_{eval}$ is indicative of $P_{test}$. Computing $P_{eval}$ estimate the time of the training for which the model best generalizes.



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{buffer_figures/error.png}
    \caption{The 3 training regimes on a regularization task. (left) the model in red yields high errors both on the train and test experience: the model is undertrained; (middle) the model fits well both the train and test experience; (right) the model fits perfectly well the train experience but not the test experience}
    \label{fig:my_label}
\end{figure}

\paragraph{Different types of experience $E$: supervised learning VS. reinforcement learning}

Experience $E$ can be collected in several manner, leading to different learning techniques. In this chapter, we introduce two learning techniques that correspond to two types of experience: supervised learning where a model is passively exposed to experience and reinforcement learning where the agent actively collect its experience.

\begin{itemize}
    \item In \textbf{supervised learning (SL)}, the model is fed and trained with labeled examples, where the correct output is provided for each example in the training data. The model is therefore passively exposed to the experience $E$. The goal of supervised learning is then to make predictions on new, unseen examples that are drawn from the same distribution as the training data. 
    \item In \textbf{reinforcement learning (RL)}, the model learns to take actions in an environment in order to maximize a reward. In reinforcement learning, the algorithm is not given explicit feedback on each action it takes, but instead must learn to optimize its behavior through trial-and-error. In that sense, the model collects its own experiences (actions and their corresponding rewards) based on the previous rewards it received. Hence, it belongs to the family of sequential decision-making methods. %Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}. It is now a promising approach to model how agents may learn to iteratively shape their language by trial-and-error experiments
\end{itemize}

Both of those approaches are inspired from how humans and animals learn. \mathieu{TO DO SL}. Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}.
\\
These learning approaches are promising to model how agents may learn to shape and use languages.

\subsubsection{Optimizing Lewis games with machine learning}

Let's now describe the optimization of the Lewis Game with machine learning algorithms. 

\paragraph{Notations} Let's denote $s$ a state taken from the state space $\mathcal{S}$. The sender $f^{\mathrm{sender}}_{\theta}$ is a neural network parameterized by $\theta$. The sender is a state-dependent probability distribution over messages $m$ belonging to the message space $\mathcal{M}$. As such, the sender maps the states (inputs) into messages (outputs):

\begin{align*}
    f^{\mathrm{sender}}_{\theta}: \mathrm{states} \to \mathrm{messages}
\end{align*}



\begin{align*}
    f^{\mathrm{receiver}}_{\phi}: \mathrm{messages} \to \mathrm{actions}
\end{align*}

%Two players are involved: the sender and the receiver. Both of them have to solve a communica-
%tion task in an environment. The environment is characterized at each time by a state. While the
%sender has access to the state, the receiver cannot observe it. A play of the game is composed of the
%following steps:
%• The sender sends a message to the receiver to communicate about the state
%2
%• The receiver chooses an action based on the message
%• Receiver’s action gives rise to a reward that depends on the combination state-act. The reward
%s then cooperatively shared between the agents.



\textit{Example}

\paragraph{What performance $P$ ?}

\textit{Example}

\paragraph{Optimization of  the sender}

\paragraph{Optimization of the receiver}

\paragraph{Tricks}





\paragraph{Different types of experience $E$: supervised learning VS. reinforcement learning}

Experience $E$ can be collected in several manner, leading to different learning techniques. In this chapter, we introduce two learning techniques that correspond to two types of experience: supervised learning where a model is passively exposed to experience and reinforcement learning where the agent actively collect its experience.

\begin{itemize}
    \item In \textbf{supervised learning (SL)}, the model is fed and trained with labeled examples, where the correct output is provided for each example in the training data. The model is therefore passively exposed to the experience $E$. The goal of supervised learning is then to make predictions on new, unseen examples that are drawn from the same distribution as the training data. 
    \item In \textbf{reinforcement learning (RL)}, the model learns to take actions in an environment in order to maximize a reward. In reinforcement learning, the algorithm is not given explicit feedback on each action it takes, but instead must learn to optimize its behavior through trial-and-error. In that sense, the model collects its own experiences (actions and their corresponding rewards) based on the previous rewards it received. Hence, it belongs to the family of sequential decision-making methods. %Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}. It is now a promising approach to model how agents may learn to iteratively shape their language by trial-and-error experiments
\end{itemize}

Both of those approaches are inspired from how humans and animals learn. \mathieu{TO DO SL}. Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}.
\\
These learning approaches are promising to model how agents may learn to shape and use languages.





\subsubsection{Optimizing a machine learning problem}

\paragraph{Measuring the performance $P$: the loss function}

\mathieu{Partir de la notion générale de loss et aboutir à l'optim de reward dans notre pb}

In order to make a neural network learn, a score measuring the success of the task should be defined. This score is called the \textit{loss function} $\mathcal{L_{\theta}}$. Note that the loss function is averaged on the experience $E$ ($\mathcal{L}_{\theta} = \mathbb{E}_{E}l_{\theta}$). The goal of training a model is then to find the set of model parameters $\theta$ that minimize the loss function given the experience $E$:

\begin{align}
    \min_{\theta} \mathcal{L}_{\theta}
    \label{eq:min_pb}
\end{align}


The choice of a loss function depends on the specific task that the model is being trained for. For example, in a classification task (e.g. object selection, attribute reconstruction), the loss function might measure the difference between the predicted class probabilities and the true class labels. In a regression task (e.g. pixel reconstruction), the loss function might measure the difference between the predicted values and the true values. The specific form of the loss function is key as it has a significant impact on the performance of the trained model.

\paragraph{Learning to optimize the performance $P$: the gradient descent}

For a computer program $f_{\theta}$, learning means improving with respect to to the optimization problem \ref{eq:min_pb}. Among all the ways of performing this optimization problem, \textit{gradient descent} methods are the most successful approaches. The gradient descent is an iterative optimization algorithm that attempts to find the minimum of a function by following the negative gradient of the function. The model parameters $\theta$ are updated at each iteration in the direction that reduces the value of the loss function. The size of the update is determined by a hyperparameter called the learning rate. The update is written: 

\begin{align}
    \theta_{n+1} = \theta_{n} - \eta \nabla_{\theta}\mathcal{L}_{\theta}(\theta_{n})
\end{align}

where $\theta_{n}$ is the model parameters at step $n$, $\theta_{n+1}$ is the model parameters at step $n+1$, $\nabla_{\theta}\mathcal{L}_{\theta}$ the gradient of $\mathcal{L}$ and $\eta$ the learning rate.

In practice, this variants of the gradient descent are used: first, computing the gradient of the averaged loss function $\nabla_{\theta}\mathcal{L}_{\theta}$ is not tractable as it would require to estimate to compute the loss function over the entire dataset. \textit{Stochastic gradient descent} tackles this issue by estimating the gradient of the loss function over a limited number of samples, a \textit{batch} of data. The batch size should be not too large to ensure a fast training, and not too small to be a correct estimate of the true gradient.

\begin{leftbar}
\textbf{}
\end{leftbar}

% \begin{leftbar}
% Using gradient descent yields several challenges:

% \begin{itemize}
%     \item \textbf{Estimating the gradient}: In practice, computing the gradient $\nabla_{\theta}\mathcal{L}_{\theta}$ at every step is impossible as it would require to compute the error over all the experience $E$. In practice, we tackle this issue by using the \textit{stochastic gradient descent} which is a variant a gradient descent for which the gradient $\nabla_{\theta}\mathcal{L}_{\theta}$ is approximated at each step using a small subset, called batch, of the experience $E$. This batch should be large enough to ensure that the estimated gradient fairly approximates the true gradient $\nabla_{\theta}\mathcal{L}_{\theta}$. The practitioner should tune the size of the batch.
%     \item \textbf{Adjusting the learning rate}: The learning rate $\eta$ controls the amplitude of the update at each step. Training dynamics are largely impacted by the choice of this parameter. Qualitatively, $\eta$ can be interpreted as a resolution parameter. On the one hand, if $\eta$ is too small, the algorithm captures very small variations of the loss function. However, the training is very slow as $\theta_{n+1}$ will be very close to $\theta_{n}$ for each iteration. On the other hand, if $\eta$ is too big, the training is fast but the algorithm cannot capture fine variations of the loss function and the estimation of model parameters minimizing $\mathcal{L}_{\theta}$ is imprecise. In practice, practitioners get ride of this issue by using the \textit{Adam optimizer} which is a variant of stochastic gradient descent that uses an adaptive learning rate, which means that the learning rate is automatically adjusted based on the dynamics of the training. 
% \end{itemize}
% \end{leftbar}

\paragraph{Different types of experience $E$: supervised learning VS. reinforcement learning}

Experience $E$ can be collected in several manner, leading to different learning techniques. In this chapter, we introduce two learning techniques that correspond to two types of experience: supervised learning where a model is passively exposed to experience and reinforcement learning where the agent actively collect its experience.

\begin{itemize}
    \item In \textbf{supervised learning (SL)}, the model is fed and trained with labeled examples, where the correct output is provided for each example in the training data. The model is therefore passively exposed to the experience $E$. The goal of supervised learning is then to make predictions on new, unseen examples that are drawn from the same distribution as the training data. 
    \item In \textbf{reinforcement learning (RL)}, the model learns to take actions in an environment in order to maximize a reward. In reinforcement learning, the algorithm is not given explicit feedback on each action it takes, but instead must learn to optimize its behavior through trial-and-error. In that sense, the model collects its own experiences (actions and their corresponding rewards) based on the previous rewards it received. Hence, it belongs to the family of sequential decision-making methods. %Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}. It is now a promising approach to model how agents may learn to iteratively shape their language by trial-and-error experiments
\end{itemize}

Both of those approaches are inspired from how humans and animals learn. \mathieu{TO DO SL}. Reinforcement learning originates from research in animal psychology with the seminal work of~\citet{thorndike1898animal} and~\citet{skinner1938behavior}. The authors studied how animals could be conditioned through trial-and-error experiments. The goal was to enforce a specific behavior by either giving positive or negative stimuli to the animals. This training intuition was later cast as a mathematical problem with dynamic programming~\citep{bellman1957dynamic,bertsekas1996neuro,puterman2014markov}, and reinforcement learning~\citep{sutton1998introduction}.
\\
These learning approaches are promising to model how agents may learn to shape and use languages.

\paragraph{Learning from experience $E$: the generalization issue} Previously presented tools allow to optimize the performance $P$ when experiencing $E$ during the training. However, this performance score on the training experience is not necessarily indicative of the performance on new, unseen experience. It is thus necessary to distinguish (1) the training experience $E_{train}$ and the corresponding performance $P_{train}$ of the model on $E_{train}$, (2) the test experience $E_{test}$ and the corresponding performance $P_{test}$ of the model on $E_{test}$. $P_{test}$ indicates how well the model generalizes. In standard machine learning training, 3 regimes are observed:

\begin{itemize}
    \item \textbf{Underfitting}: When the model is undertrained, it is unable to have good performance $P$ neither on the training and test experience. $P_{train}$ and $P_{test}$ are bad.
    \item \textbf{Generalization}: During training, there is a time when both the both $P_{train}$ and $P_{test}$ are good. It may not be the optimal performance $P_{train}$ that could be achieved on $E_{train}$ but it is a good compromise to generalize well.
    \item \textbf{Overfitting}: When the model is overtrained, it reaches very good performances $P_{train}$ on $E_{train}$ but performances $P_{test}$ on $E_{test}$ are bad: the model overfits on the training experience.
\end{itemize}

The main challenge of machine learning is to find the right balance between under and overfitting to reach the generalization regime. Several methods are commonly used including regularization techniques and early stopping, which consists in introducing an evaluation experience $E_{eval}$ for which the performance $P_{eval}$ is indicative of $P_{test}$. Computing $P_{eval}$ estimate the time of the training for which the model best generalizes.



\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\textwidth]{buffer_figures/error.png}
    \caption{The 3 training regimes on a regularization task. (left) the model in red yields high errors both on the train and test experience: the model is undertrained; (middle) the model fits well both the train and test experience; (right) the model fits perfectly well the train experience but not the test experience}
    \label{fig:my_label}
\end{figure}


% Rosenblatt (1958) perceptron with learnable weights (perceptron)
% Minsky and Papert 1969 ;
% LeCun et al. 1985 and Rumelhart et al. 1986 => train multilayer perceptrons thourgh BP
% Then winter of ML because of blackbox
% Hinton Bengio LeCun 2006 tricks and to practically and reliably train deep multi-layer networks
% Dahl et al 2010 and Hinton et al 2012 => breakthgough in speeck
% Krizhevsky AlexNet 2012 and He et al. 2016 Resnet 2016 
% Mnih et al. 2013 (Atari) et Silver 2016 Deep RL (AlphaGo)



% 

\subsection{\mathieu{OLD} Opportunity and challenges regarding the simulation of language emergence}

Machine learning simulations provide an opportunity to explore more realistic scenarios by creating more challenging tasks and scaling up the simulations. However, the usefulness of these simulations is conditioned on a clear understanding of the simulations and the ability to compare human and artificial languages.

\subsubsection{Toward more realistic language evolution scenarios}

Machine learning simulations provide a powerful tool for modeling crucial aspects of human language and communication. These simulations can capture the ability to coordinate effectively within a group, the intricate interplay between language and other modalities, the functional role of language in communication, etc.

\paragraph{More realistic dynamic scenarios} Researchers are exploring ways to create more realistic scenarios in dynamic environments to design language evolution scenarios using machine learning. A first approach is to question the way communication is modeled. For instance, \cite{evtimova2017emergent,Valentin} attempt to extend symbolic communication to conversations in multi-turn referential games, while \cite{bullard2020exploring} explore nonverbal communication using spatially articulated agents. A second approach aims at grounding agents in more realistic environments and study tasks that go beyond referential tasks. Early studies focused on how agents communicate about visual inputs~\citep{lazaridou2016multi}, while more recent studies~\citep{das2019tarmac}, immerse agents in realistic 2D and 3D environments to investigate how they use communication to solve navigation tasks. Additionally, \cite{jaques2019social} examine social dilemma environments and communication as a means of influence between agents.

\paragraph{Scaling  experiments} Most of human and agent-based simulations are constrained in terms of scale across various aspects of the game, such as the number of participants, generations, and task complexity. \mathieu{cites}. Neural network simulations provides the opportunity to extend these parameters to an unprecedented scale, which is essential in simulating realistic evolutionary scenarios. 
\cite{chaabouni2022emergent} examine two scaling procedure. They scale the difficulty of the visual discrimination game (see Sec. \ref{sec:case_study}) by both working with large image datasets of millions of images and tasking the receiver to discriminate an image among a set of thousands of candidates. Agents should then build a referential system that can cope with the complexity of the task. They also scale they build populations of a size that goes up to $100$ agents. Another bunch of works \mathieu{cites} study generational transmission up to \mathieu{X} generations. Human or pre-neural network simulations have never reached this scale neither in term of task complexity, number of paricipants of number of generations.

% Scaling in time ; % Scaling in  space

% Foester 2016
% Multi-turn Evtimova , Valentin & Paul
% Visually grounded Das
% emboddied kalesha
% Ecological situations - Natasha Jaques et al.
% Doesn't go without issues -> Lowe et al. 2019 Pitfall of measuring comm

% Large Scale (socio-cultural constraints) - Chaabouni et al. 2022 + Carroll 2019


\paragraph{Incorporating recent breakthrough in language modeling into language evolution simulations} 

\mathieu{TO DO RAHMA}

\mathieu{papiers récents d'Angeliki + tutorial + ajout récent}
\mathieu{Rq. inclure diplomacy}
\mathieu{rq. sur GPT + chatGPT}

%%%%%%%%%%%%%%%%%%%%%%%%%% EN COURS D ECRITURE %%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Challenges} 
% 1. Agent design
% 2. Comparing human and artificial comm
% 3. Emerging comm

\paragraph{Agents design} Designing agents remains a core challenge of language emergence simulations~\citep{galke2022}.
%
First, in most neural emergent communication, agents are either senders or listeners. However, in human simulations, participants alternate between these two roles~\citep{kirby2015compression,raviv2019larger}. The idea behind this approach is that a participant should reproduce the messages it understands~\citep{hockett1960origin}. The main issue related to role alternation is modeling the interplay between comprehension and production which is a complex topic in cognitive science. Comprehension and production could stem from the same mental processes and activate the same neurons in the brain \citep{pickering2004toward}. An alternative viewpoint is that comprehension and production are distinct processes that rely on different neural networks. In this case, the production and comprehension of language are separate but still interconnected through the shared experience of using language. In neural network simulations, this raises the question on how building the interplay between understanding and generation modules. \cite{graesser2019emergent} design a symmetric agent with a core module from which derive both the understanding and production modules meaning that neurons/weights are shared between the two modalities. \mathieu{Paul} use a partitioning training method to ensure that any agent is self-consistent, meaning it comprehends all the messages it generates.

%
Second, neural networks are over-parameterized with respect to the tasks studied. The consequence is that neural agents can learn and memorize a large amount of knowledge. For instance, \mathieu{Michel, Rita} have shown that when playing a population-based referential game, receivers can simultaneously learn multiple languages from different senders This presents a challenge in terms of agent modeling. On the one hand, the capacity of human memory is one of the most significant limitations in language learning~\citep{galke2022}, which plays a vital role in explaining how language structures emerge across generations and through the effect of group size. \cite{resnick2019capacity} actually demonstrated that constraining neural agents capacity can facilitate the emergence of compositionality.
% gen Cornish 2017 ; group size Meir et al 2012 Wray and Grace 2007
On the other hand, it has also been shown that generational transmission and group size effects can occur only without any memory constraints but through playing with optimization constraints \mathieu{cites}.
% Remark sur le fait que tout passe par le scale


%%%% METRICS %%%%%

\paragraph{Comparing human and artificial languages} 
%
As discussed above, the comparison between human and artificial languages lie on a transposition of language universals into quantitative metrics. This transposition raises several issues. 
% consistency of universals across levels
First, human languages are composed of several linguistic levels with different structural properties. In particular, there is a dual articulation in language \mathieu{ref}: languages are composed of two combinatorial systems, a sub-lexical one at the level of phonemes or characters that are combined to produce an infinite number of words or morphemes, a supra-lexical one at the level of words or phonemes that are combined to produce compositional meanings. These two combinatorial systems do not have the same properties and particularly, studying compositionality only make sense at the supra-lexical level. However, in neural artificial languages, compositionality is only computed at the level of message symbols which is the lowest linguistic unit.
% the weak transposition of human concepts to artificial languages 
Second, 
% 

However, human and artificial languages are different objects: human languages are hierarchical structures with different linguistic levels while artificial languages are sequential probabilistic distributions. I


Comparing human and nonhuman communication is a long-standing challenge~\citep{raviv2022simple} \mathieu{cites}. Similarly, evaluating artificial languages raises several issues. 

% 
%
%
%
%

First, human language universals are abstract properties whose evaluation is quantified across a large number of factors whose measurements vary across communities. 
% level

% + la question des distances wrt dependency trees
%\bigbreak 
% Second: the notion of scale Example de compo
%Second, some works concentrate on comparing human and artificial languages using metrics tailored to artificial languages, i.e. probabilistic distributions. Such metrics include information theory based metrics \mathieu{cites} such as entropy \mathieu{cites}. While, such metrics start 

% First: partir des humains vers les langues artificiels = identify languages universals / take human languages metrics  

\paragraph{Issues when working in realistic scenarios} When moving from a referential 
% issues with scaling
% issues with complex environments => measure

While machine learning simulations open the opportunity to build complex environments where a population of agents interact with their environment and communicate between each other, it also opens question on measuring if communication protocols emerge. \cite{lowe2020interactionx}


\subsubsection{Approaches in comparing neural and human languages}
\label{subsubsec:metrics}

We here present standard approaches for comparing neural and human languages. 

% When comparing neural emergent and human languages we need to clarify:
% \begin{itemize}
%     \item \textbf{What is a neural emergent language ?} Once the task optimized by the agents is solved, Sender agents map structured sets, namely the environment observations $x$, to sequences of discrete symbols, namely the messages $m$. These mappings $x \to m$ are referred to as a neural emergent languages.
%     \item \textbf{What is a natural language ?} Raising universal properties of human languages is a difficult task because languages are as different as they are alike. When comparing natural and artificial languages, the main approach is to focus on language universals or trends that are shared across all languages. 
% \end{itemize}

% Two main group of properties that are used to compare artificial and natural languages:

% \mathieu{Difficulté à distinguer les métriques qu'on peut compute pour comparer les deux / les trends global (iterated learning + demographic trends)}

% Intepre (semantic categorization)
\paragraph{Qualitative interpretation of semantic conceptualization ?} Once a task solved, Sender agents map environment observations $x$, to sequences of discrete symbols $m$. Neural emergent languages are precisely those mappings $x \to m$. A first approach to compare neural and human languages is to evaluate the interpretability of messages in relation to human semantic categories. Qualitative methods can be used to determine if symbols in messages can be linked to certain features of environment observations, such as the labels of images~\citep{lazaridou2016multi,chaabouni2022emergent,dessi2021interpretable}.
% Structural properties ; universals ; Compositionality + generaliazation (combinatorial property)
\paragraph{Quantitative measures of languages universals} Human languages can be described in terms of universals, i.e. abstracts properties that are found across all human languages. The origin of these universals is still the subject of many research questions in linguistics and cognitive science, and more recently machine learning with the emergent communication framework. We review here the most studied language universals in this framework:
\begin{itemize}
    \item \textbf{Compositionality} It refers to the ability to decompose the meaning of an utterance as a function of its constituents~\citep{hockett1960origin}. Compositionality arouses a lot of interest in the deep learning community because it is considered as a prerequisite for generalization~\citep{kottur2017natural,cogswell2019emergence}. Neural emergent communication literature~\citep{lazaridou2018emergence} \mathieu{REF} reintroduced topographic similarity~\citep{brighton2006understanding} which  captures the systematic relation between meanings and forms~\citep{lazaridou2020emergent}. To this end, it computes the correlation between pairwise observations distances and the corresponding message distances. As topographic similarity depends on the chosen distances in the observation and meaning spaces, other metrics have been introduced in the literature, such as disentanglement~\citep{chaabouni2020compositionality}, or Tree Reconstruction Error~\citep{andreas2019measuring}.
    %
    \item \textbf{Efficiency} Human languages efficiently encode information. This efficiency has been observed in multiple levels. The emergent communication literature mainly studied the efficiency of natural languages in term of word length and semantic categorization. For the former, \citep{chaabouni2019anti, rita2020lazimpa} have looked at the Zipf’s Law of Abbreviation\citep{zipf1949principie}, whereas \citep{chaabouni2021communicating, tucker2022towards} studied how artifical neural agents use color naming systems to partition the colors into efficient semantic categories. In both cases, these studies have used metrics introduced in the cognitive science domain~\citep{zipf1949principie, Regier2015}

    %
    \item \textbf{Word order/case marking} Across human languages, linguists observed this inverse correlation between the use of case and the use of fixed word order to disambiguate words’ role in sentences\citep{Comrie:1981, Blake:2001, Sinnemaki:2008}. That is, languages with freer word order tend to use explicit grammatical marking (e.g., Japanese), whereas languages with more fixed word order rarely rely on case-marking (e.g., English). Some work in the machine learning framework investigated the origin of this trade-off by looking at the evolution of artificial languages~\citep{lian2023communication, chaabouni2019word}.

    \item \textbf{Demographic trends} As experiments with neural networks can now involve many agents, researchers are trying to replicate demographic trends observed in language evolution, such as the impact of population size on language structures~\citep{Nettle2012,Bromham2097,Reali2018,raviv2019larger}. Many studies have shown a correlation between population size and various language features, with larger communities tending to develop simpler grammars~\citep{Lupyan2010,meir2012influence,WALS,Reali2018,raviv2019larger}. Possible explanations for this correlation include the variation of the proportion of contact agents~\citep{wray2007543,clyne1992linguistic}, the proportion of second learners~\citep{ellis2008dynamics}, or changes in network topology~\citep{wagner2009communication}. All of those parameters can be controlled in neural emergent communication.
\end{itemize}
